Automatically Locating ARM Instructions Deviation between Real Devices and CPU Emulators

Emulator is widely used to build dynamic analysis frameworks due to its fine-grained tracing capability, full system monitoring functionality, and scalability of running on different operating systemsand architectures. However, whether the emulator is consistent with real devices is unknown. To understand this problem, we aim to automatically locate inconsistent instructions, which behave differently between emulators and real devices. We target ARM architecture, which provides machine readable specification. Based on the specification, we propose a test case generator by designing and implementing the first symbolic execution engine for ARM architecture specification language (ASL). We generate 2,774,649 representative instruction streams and conduct differential testing with these instruction streams between four ARM real devices in different architecture versions (i.e., ARMv5, ARMv6, ARMv7-a, and ARMv8-a) and the state-of-the-art emulators (i.e., QEMU). We locate 155,642 inconsistent instruction streams, which cover 30% of all instruction encodings and 47.8% of the instructions. We find undefined implementation in ARM manual and implementation bugs of QEMU are the major causes of inconsistencies. Furthermore, we discover four QEMU bugs, which are confirmed and patched by thedevelopers, covering 13 instruction encodings including the most commonly used ones (e.g.,STR,BLX). With the inconsistent instructions, we build three security applications and demonstrate thecapability of these instructions on detecting emulators, anti-emulation, and anti-fuzzing.

==> tables/random_testcases.tex <==
\begin{table*}[]
\footnotesize
\caption{\small{The statistics of the generated instructions in random. "Max" denotes maximum value. "Min" denotes minimum value. "Ave" denotes average value. For each instruction set and the overall result, "Ratio" inside column "VIS", "CE", "CI", and "Covered Constraints" denotes the percentage of dividing "Ave" inside the same column by "VIS", "CE", "CI", and "Solved Constraints" in Table~\ref{tab:testcase}, respectively. “VIS”, "CE", "CI" denotes the same meaning illustrated in Table~\ref{tab:testcase}.}
}

\begin{tabular}{cc|cccc|cccc|cccc|cccc}
\toprule
Instruction  & Generated & \multicolumn{4}{c|}{VIS} & \multicolumn{4}{c|}{CE} & \multicolumn{4}{c|}{CI} & \multicolumn{4}{c}{Covered Constraints} \\ \cline{3-18} 
                           Set & Instruction     & Max     & Min     & Ave    &
                   Ratio &              Max     & Min    & Ave    &
                   Ratio &  
                   Max     & Min    & Ave &    
                   Ratio &  
                   Max     & Min    & Ave &    
                   Ratio 
                   \\ \hline
                    \hline
A64             &1,094,700                 & 422,431      & 420,949      & 421,645  & 38.5    & 273         & 261         & 265   &31.6  &189 & 174& 178& 30.6  & 955          & 923         & 934    & 27.2     \\ \hline
A32            &870,221                  & 579,602      & 577,723      & 578,845  & 66.5     & 420         & 409         & 415   & 75.5    & 365 & 356& 361& 75.1 & 3772         & 3665        & 3725   &  79.0   \\ 
T32          &808,770                    & 34,882       & 34,298       & 34,598  & 4.2     & 356         & 348         & 351   &  66.1  & 287 & 278 & 283 & 62.7  & 3246         & 3178        & 3203   &  72.3    \\
T16            &958                  & 806         & 782         & 796  &   83.0    & 61          & 55          & 57  & 73.1    &52 & 47& 49&  72.1  & 94           & 79          & 84     &   68.9   \\ \hline 
Overall & 2,774,649 & 1,037,721 & 1,033,752 & 1,035,884 & 37.3 & 1,110 & 1,073 & 1,088 & 54.5 & 560 & 542&  550& 51.4 & 8,067 & 7,845 & 7,946 & 62.6 \\ 

\bottomrule
\end{tabular}
\label{tab:random_testcase}
\end{table*}

==> tables/symbolic_execution.tex <==
\begin{table}[]
\footnotesize
\caption{\small{The detailed steps to solve the constraint \code{$d4 > 4$}.}}

\begin{tabular}{ccc}
\toprule
\begin{tabular}[c]{@{}c@{}}Original \\ Expression\end{tabular} & \begin{tabular}[c]{@{}c@{}}Execute \\ Statement\end{tabular} & \begin{tabular}[c]{@{}c@{}}New \\ Expression\end{tabular} \\ \hline \hline
d4 \textgreater 31                                             & d4 = d3 + inc                                                & d3 + inc \textgreater 31                                  \\ 
d3 + inc \textgreater 31                                       & d3 = d2 + inc                                                & d2 + 2*inc \textgreater{}31                               \\ 
d2 + 2*inc \textgreater 31                                     & d2 = d + inc                                                 & d + 3*inc \textgreater{}31                                \\ 
d + 3*inc \textgreater{}31                                     & d = UInt(D:Vd)                                               & Vd + 16*D + 3*inc \textgreater 31                         \\ \bottomrule
\end{tabular}
\label{tab:se_example}
\end{table}
